Search for reactor-produced millicharged particles with Skipper-CCDs at the CONNIE and Atucha-II experiments

Millicharged particles, proposed by various extensions of the standard model, can be created in pairs by high-energy photons within nuclear reactors and can interact electromagnetically with electrons in matter. Recently, the existence of a plasmon peak in the interaction cross-section with silicon in the eV range was highlighted as a promising approach to enhance low-energy sensitivities. The CONNIE and Atucha-II reactor neutrino experiments utilize Skipper-CCD sensors, which enable the detection of interactions in the eV range. We present world-leading limits on the charge of millicharged particles within a mass range spanning six orders of magnitude, derived through a comprehensive analysis and the combination of data from both experiments.

==> fig/PRL_justification.tex <==
\section{PRL Justification}

% This analysis provides the first combined limit, based on measurements by two independent reactor neutrino experiments, on relativistic millicharged particle production by nuclear reactors. 
% Thanks to the use of extremely sensitive silicon Skipper-CCD detectors, the CONNIE and Atucha-II experiments achieve ultra-low detection thresholds, allowing to probe the lowest interaction energies of millicharged particles with atomic electrons. 
% At this energy the interaction probability is increased by a significant plasmon peak at 15 eV, enhancing greatly the experimental sensitivity to sub-MeV relativistic particles. 
% Thus, world-leading limits on the charge of millicharged particles are achieved in a mass range spanning six orders of magnitude. 
% While the individual experimental limits already improve the current best bounds, their combination provides a very robust limit that improves further the world-leading limit on millicharged particle production at reactors. 

Thanks to the use of extremely sensitive silicon Skipper-CCD detectors, the CONNIE and Atucha-II reactor neutrino experiments achieve ultra-low detection thresholds, allowing to probe the lowest interaction energies of millicharged particles with atomic electrons.  The interaction probability is increased by a significant plasmon peak at 15 eV, enhancing greatly the experimental sensitivity to sub-MeV relativistic particles. 
While the individual experimental limits already improve the current best bounds, their combination provides a very robust limit that improves further the world-leading limit on millicharged particle production at reactors in a mass range spanning six orders of magnitude. 

% \subsection{Word count}
% Text: 2305
% Math Inline: 209
% Math Display: 144
% Tables: ~430
% Figures: ~430
% 79 + 4.7/8.5 * 150 + 20 + 4/8.5 * 150 + 20 + 7.8/8.5 * 150 + 20 


\clearpage
